Multi-Domain Neural Machine Translation with Word-Level Adaptive Layer-wise Domain Mixing

Many multi-domain neural machine translation (NMT) models achieve knowledge transfer by enforcing one encoder to learn shared embedding across domains. However, this design lacks adaptation to individual domains. To overcome this limitation, we propose a novel multi-domain NMT model using individual modules for each domain, on which we apply word-level, adaptive and layer-wise domain mixing. We first observe that words in a sentence are often related to multiple domains. Hence, we assume each word has a domain proportion, which indicates its domain preference. Then word representations are obtained by mixing their embedding in individual domains based on their domain proportions. We show this can be achieved by carefully designing multi-head dot-product attention modules for different domains, and eventually taking weighted averages of their parameters by word-level layer-wise domain proportions. Through this, we can achieve effective domain knowledge sharing, and capture fine-grained domain-specific knowledge as well. Our experiments show that our proposed model outperforms existing ones in several NMT tasks.

==> tech report/abstract.tex <==
%!TEX root = ./MultiDomainNMT.tex

\begin{abstract}
	
	Many multi-domain neural machine translation (NMT) models achieve knowledge transfer by enforcing one encoder to learn shared embedding across domains. However, this design lacks adaptation to individual domains. To overcome this limitation, we propose a novel multi-domain NMT model using individual modules for each domain, on which we apply word-level, adaptive and layer-wise domain mixing.
	%\todo{'word-level multistage adaptive' is quite confusing} 
	We first observe that words in a sentence are often related to multiple domains. Hence, we assume each word has a domain proportion, which indicates its domain preference. Then word representations are obtained by mixing their embedding in individual domains based on their domain proportions.
	%We then integrate the domain proportions of the words with the transformer model. Specifically, we design multi-head attention modules for each individual domains, and then mix these modules by taking weighted averages of their parameters by the domain proportion of the word. 
	%By using adaptive domain proportions for the words,
	We show this can be achieved by carefully designing multi-head dot-product attention modules for different domains, and eventually taking weighted averages of their parameters by word-level layer-wise domain proportions.
	%We show this can be achieved by carefully designing multi-head dot-product attention modules for different domains, and eventually mixing these modules by taking weighted averages of their parameters by their layer-wise domain proportions. 
	Through this, we can achieve effective domain knowledge sharing, and capture fine-grained domain-specific knowledge as well. Our experiments show that our proposed model outperforms existing ones in several NMT tasks.
	
\end{abstract}

==> tech report/background.tex <==
%!TEX root = ./acl2019.tex

\vspace{-0.1in}
\section{Background} \label{sec:background}
\vspace{-0.1in}

\textbf{Neural Machine Translation} (NMT) directly models the conditional distribution of the translated sentence $\yb=(y_1,...,y_\ell)$ given a source sentence
$\xb=(x_1,...,x_\ell)$.\footnote{Here we assume that we have applied padding to all sentences, and therefore, they are all of the same length.}. The conditional probability density function $p(\yb|\xb)$ is parameterized by an encoder-decoder neural network: The encoder encodes the source sentence into a sequence of hidden representations $\cH(\xb) = (h_1, ..., h_n)$, and the decoder generates target sentence one token at a time using these intermediate representations. More specifically, the decoder usually contains a recursive structure for computing $p(y_t|y_{<t},\xb)$ by
\begin{align*}
p(y_t|y_{<t},\xb)= \cF(\cG_t,\cH(\xb),y_{t-1}),
\end{align*}
where $\cG_{t}$ denotes the hidden representation of the decoder for the $t$-th position of the sequence, and $\cF$ denotes a multi-layered network that outputs the probability of $y_t$. Notice that $\cG_{t}$ is generated by the $\cG_{t-1}, \cH(\xb)$, and the previous word $y_{t-1}$. Given $N$ pairs of source/target sequences denoted by $\{\xb_i, \yb_i\}_{i=1}^n$, we train the NMT model by minimizing the cross-entropy loss as follows,
\begin{align*}
	\textstyle\min_{\cH,\cG,\cF}L_{\rm gen}= \frac{1}{n}\sum_{i=1}^n -\log p(\yb_i|\xb_i)
\end{align*}
where $p(\yb_i|\xb_i) = \prod_{t=1}^mp(y_{i,t}|y_{i,<t},\xb_i)$.

\medskip

\noindent\textbf{Transformer} is one of the most popular NMT models \citep{vaswani2017attention,tubay2018neural, devlin2018bert}. The encoder and decoder in Transformer contain stacked self-attention and point-wise, fully connected layers without any explicit recurrent structure, which is different from existing RNN-based NMT models. 

%For each $y_i$, an attention weight is generated over the output embedding of the encoder. Such an attention mechanism allows the decoder to attend over a part of input that is more relevant, when generating each output token \citep{luong2015effective, bahdanau2014neural}. 
% The attention model is based on the estimation of a probability distribution over all input words for each target word. Word alignments with attention weights can then be easily deduced from such distributions and support the translation. 

Specifically, \citet{vaswani2017attention} propose a new attention function using the scaled dot-product as the alignment score, which takes the form,
\begin{align}\label{dot-product}
\mathrm{Attention}(Q,K,V)=\mathrm{softmax}\Big(\frac{QK^\top}{\sqrt{d}}\Big)V,
\end{align}
%where $Q\in \RR^{\ell \times d}$ is a matrix that contains the query (vector representation of one word in the sequence), $K\in \RR^{\ell \times d}$ are all the keys (vector representations of all the words in the sequence) and $V\in \RR^{\ell \times d}$ are the values, which are again the vector representations of all the words in the sequence.  \todo{too verbose}For the encoder and decoder, the self-attention modules, $Q$ consists of the same word sequence as $V$ and $K$. However, for the attention module that is taking into account the encoder and the decoder sequences, $Q$ is different from the sequence represented by $V$ and $K$.
where $Q,K,V\in \RR^{\ell \times d}$ are the vector representations of all the words in the sequences of queries, keys and values accordingly.  For the self-attention modules in the encoder and decoder, $Q=K=V$; For the attention module that takes into account the encoder and the decoder sequences, $Q$ is different from the sequence represented by $V$ and $K$.

\begin{figure}[!ht]
	\centering
	\vspace{-0.1in}
	\includegraphics[width=0.4\textwidth]{figure/MultiHeadAtt.png}
	\vspace{-0.2in}
	\caption{Multi-head Scaled Dot-Product Attention.}
	\vspace{-0.15in}
	\label{fig:multiheadatt}
\end{figure}

Based on the above attention function in \eqref{dot-product}, \citet{vaswani2017attention} further develop a multi-head attention module, which allows the NMT model to jointly attend to information from different representations at different positions. In particular, we consider a multi-head attention module with $m$ heads. For the $i$-th head $H_i$, three point-wise linear transformations $W_{i,Q},~W_{i,K}~,~W_{i,V}\in\RR^{d\times d/m}$ are first applied to the input $Q$, $K$ and $V$, respectively, and then the scaled dot-product attention is applied: Let $\tilde{Q}_i=QW_{i,Q}$, $\tilde{K}_i=KW_{i,K}$ and $\tilde{V}=VW_{i,V}$,
\begin{align}\label{MHT}
H_i=\textrm{Attention}(\tilde{Q}_i,\tilde{K}_i,\tilde{V}_i).
\end{align}
Eventually, the final output applies a point-wise linear transformation $W_O\in\RR^{d\times d}$ to the concatenation of the output from all heads:
\begin{align*}
\textrm{MultiHead}(Q,K,V) = \textrm{Concat}(H_1,...,H_m)W_O.
\end{align*}
An illustrative example of the multihead attention architecture is provided in Figure~\ref{fig:multiheadatt}.

In addition to the above multi-head attention modules, each layer in the encoder and decoder in Transformer contains a point-wise two-layer fully connected feed-forward network. 

==> tech report/conclusion.tex <==
%!TEX root = ./acl2019.tex
\vspace{-0.1in}
\section{Discussions} \label{sec:discussion}
\vspace{-0.1in}

One major challenge in multi-domain machine translation is the word ambiguity in different domains. For example, the word ``article'' has different meanings in the domains of laws and media. When translating ``article" into Chinese, the translated words are \begin{CJK*}{UTF8}{gbsn}
	``条款''
\end{CJK*} and \begin{CJK*}{UTF8}{gbsn}
	``文章''
\end{CJK*}, meaning a separate clause of a legal document and a piece of writing. Our proposed word-level layer-wise domain mixing approach tends to reduce the word ambiguity. As mentioned in Section~\ref{sec:layerwise}, our model extracts different representations of each word from contexts at different layers. Accordingly, the domain proportion of each word evolves from bottom to top layers, and can eventually help identify the corresponding domains.

\begin{table}[!htb]
	\centering
	\begin{tabular}{ c|c } 
		\hline
		\multirow{2}{*}{Laws} & ``\textbf{Article} 37 The freedom of marriage ...'' \\
		& \begin{CJK*}{UTF8}{gbsn}
			``第三十七\textbf{条}:婚姻的自由 ...''
		\end{CJK*} \\
		\hline
		\multirow{2}{*}{Media}& ``... working on an \textbf{article} about the poems ...'' \\
		& \begin{CJK*}{UTF8}{gbsn}
			``... 为了一篇诗的\textbf{文章} ...''
		\end{CJK*}\\
		\hline
	\end{tabular}
	\caption{The ambiguity of ``articles''.}
\end{table}

Moreover, as mentioned in Section~\ref{sec:word_level_mixing}, the positional embedding also contributes to the word disambiguation in multi-domain translation. For example, in the law domain, we find that ``article'' often appears at the beginning of a sentence, while in the media domain, the word ``article'' may appear in other positions. Therefore, varying domain proportions for different positions can help with word disambiguation.

We remark that word disambiguation across domains actually requires $\cD(x)$ to be powerful for predicting the domain of the word. However, a powerful $\cD(x)$ tends to yield skewed domain proportions and is not flexible enough for domain knowledge sharing. To trade off between strength and flexibility of $\cD(x)$, the smoothing parameter $\epsilon$ of $\cD(x)$ (see Section~\ref{sec:domainprop}) needs to be properly set.

\vspace{-0.1in}
\section{Conclusions} \label{sec:conclusion}
\vspace{-0.1in}

We present a novel multi-domain NMT with word-level layer-wise domain mixing, which can adaptively exploit the domain knowledge. Unlike the existing work, we construct multi-head dot-product modules for each domain and then combine them by the layer-wise domain proportion of every word. The proposed method outperforms the existing embedding based methods. We also show mixing method can be combined with embedding based methods to make further improvement. 

Moreover, we remark that our approach can be extended to other multi-domain or multi-task NLP problems. We will also investigate how to apply our approach to more complex architectures, e.g., pre-trained BERT encoder \citep{devlin2018bert}. 


==> tech report/experiment.tex <==
%!TEX root = ./acl2019.tex

\vspace{-0.1in}
\section{Experiment} \label{sec:exp}
\vspace{-0.1in}

%\subsection{Datasets}
We conduct experiments on three different machine translation tasks: %English-to-German, English-to-French and Chinese-to-English.
\smallskip

\noindent$\bullet$ \textbf{English-to-German}. We use a dataset from two domains: News and TED. We collect the News domain data from Europarl \citep{koehn2005europarl} and the TED domain data from IWLST \citep{cettolo2014report}.

\smallskip

\noindent$\bullet$ \textbf{English-to-French} We use a dataset containing two domains: TED and Medical domain. We collect TED domain data from IWLST \citep{cettolo2017overview} and medical domain data from Medline \citep{yepes2017findings}. %The data in two domains is imbalanced as well, but we do not perform downsampling for this dataset.

\smallskip

\noindent$\bullet$ \textbf{Chinese-to-English} We use a dataset containing four domains: News, Speech, Thesis and Laws. We collect the Laws, Speech, and Thesis data from UM-Corpus \citep{tian2014corpus}, and the News data from LDC \citep{openldc}. The translation from Chinese-to-English is inherently difficult. The four-domains setting makes it even more challenging. This dataset is also used in \citet{zeng2018multi}.

\smallskip

The sizes of training, validation, and testing sets for different language pairs are summarized in Table~\ref{tab:data}. We tokenize English, German and French sentences using MOSES script \citep{koehn2007moses} and perform word segmentation on Chinese sentences using Stanford Segmenter \citep{tseng2005conditional}. All sentences are then encoded using byte-pair encoding \cite{sennrich2015neural}. We evaluate the performance using two metrics: BLEU \cite{papineni2002bleu} and perplexity following the default setting in fairseq with beam search steps of $5$. 


\begin{table}[!hbt]
	\centering
	\small
	\vspace{-0.05in}
	\begin{tabular}{c|cccc}
	    \hline
		\textbf{Language} & \textbf{Domain} & \textbf{Train} & \textbf{Valid} & \textbf{Test}  \\
		\hline
		\hline
		\multirow{2}{*}{\textbf{EN-DE}} 
		& News & 184K & 18K & 19K  \\
		& TED & 160K & 7K & 7K  \\
		\hline
		\multirow{2}{*}{\textbf{EN-FR}} 
		& TED & 226K & 10K & 10K  \\
		& MEDICAL & 516K & 25K & 25K  \\
		\hline
		\multirow{4}{*}{\textbf{ZH-EN}} 
		& Laws & 219K & 600 & 456  \\
		& News & 300K & 800 & 650  \\
		& Speech & 219K & 600 & 455  \\
		& Thesis & 299K & 800 & 625  \\
	    \hline
	\end{tabular}
	\vspace{-0.1in}
	\caption{The numbers of sentences in the datasets.}
	\vspace{-0.15in}
	\label{tab:data}
\end{table}



\vspace{-0.1in}
\subsection{Baselines} 
\vspace{-0.1in}

Our baselines include the Transformer models trained using data from single and all domains. We also include several domain aware embedding based methods, which train the embedding of the encoder along with domain information. 

\smallskip

\noindent $\bullet$\textbf{Multitask Learning (MTL)} proposed in \citet{britz2017effective} uses one sentence-level domain classifier to train the embedding. Note that their classifier is only used to predict the domain, while our model uses multiple word-level domain classifiers to obtain the domain proportions for different layers (further used for domain mixing). %We use the same attention based domain classifier as they proposed.

\smallskip

\noindent $\bullet$ \textbf{Adversarial Learning (AdvL)} proposed in \citet{britz2017effective} is a variant of MTL, which flips the gradient before it is back-propagated into the embedding. This encourages the embedding from different domains to be similar.

\smallskip

\noindent $\bullet$ \textbf{Partial Adversarial Learning (PAdvL)} To combine the advantages of the above two methods, we split the embedding into half of multitask part and half of adversarial part. 

\smallskip

\noindent $\bullet$ \textbf{Word-Level Domain Context Discrimination (WDC)} \citet{zeng2018multi} integrates MTL and AdvL with word-level domain contexts. This method requires the dimension of the embedding to be doubled and, thus, is not directly applicable in Transformer. We use a point-wise linear transformation to reduce the dimension.

Moreover, \citet{zeng2018multi} consider the word-level domain aware weighted loss (\textbf{WL}). Specifically, they assign a domain-aware attention weight $\beta_j$ to the $j$-th position in the output sentence, and the corresponding weighted loss is:
\[
\textstyle L_{\textrm{gen}} = -\frac{1}{n} \sum_{j=1}^n (1+\beta_j) \log p(y_j | \xb, y_{<j}). \]
Here $\beta_j$ is obtained by an attention based domain classifier built upon the last hidden layer. 

\vspace{-0.075in}
\subsection{Details of Our Implementation} \label{sec:implementation_details}
\vspace{-0.075in}

All of our experiments are conducted under fairseq \citep{ott2019fairseq} environment. We follow the fairseq re-implementation of Transformer designed for IWLST data. Specifically, the re-implementation of Transformer differs from \citet{vaswani2017attention} in that the embedding dimension is $512$ for both the encoder and decoder, the number of heads is $6$, and the embedding dimension in the feed-forward layer is $1024$. In terms of the optimization, we follow the training recipe provided by fairseq. Specifically, we use Adam optimizer \citep{kingma2014adam} with $\beta_1=0.9, \beta_2=0.98$ with a weight decay parameter of $10^{-4}$. The learning rate follows the inverse square root schedule \cite{vaswani2017attention} with warm-up steps of $4000$, initial warm-up learning rate of $10^{-7}$, and the highest learning rate of $5 \times 10^{-4}$. For effective training, $L_{\textrm{gen}}$ is replaced by a label-smoothing cross-entropy loss with a smoothing parameter of $0.1$ \cite{szegedy2016rethinking}. 

For our domain mixing methods, we set the smoothing parameter $\epsilon$ of the domain proportion as $0.05$. Besides applying domain mixing to both the encoder and decoder (\textbf{E/DC}), we consider applying domain mixing to only the \textbf{Encoder}. The domain proportion layers $\cD$ are only used for estimating the domain proportion and should not intervene in the training of the translation model. So the gradient propagation is cut off between the Transformer and the domain proportion as Figure~\ref{fig:detached_train} shows. More discussion about the training procedure can be found in Section~\ref{sec:grad_flow}.
\begin{figure}[!htb]
	\centering
	\vspace{-0.15in}
	\includegraphics[width=0.3\textwidth]{figure/detached_train.png}
	\vspace{-0.15in}
	\caption{Computational graph for training the domain proportion layers.}
	\vspace{-0.15in}
	\label{fig:detached_train}
\end{figure}

\vspace{-0.075in}
\subsection{Experimental Results} 
\vspace{-0.075in}

Table~\ref{tab:en2deExp} shows the BLEU scores of the baselines and our domain mixing methods for English-to-German translation. As can be seen, our methods outperform the baselines on both domains. 

\begin{table}[!hbt]
\vspace{-0.1in}
    \centering
%    \small
    \begin{tabular}{c|c|c}
    \hline
    Method & News & TED  \\
    \hline
    \hline
    \multicolumn{3}{c}{Direct Training}\\
    \hline
    News & 26.09& 6.15\\
    TED & 4.90& 29.09\\
    News + TED & 26.06& 28.11\\
    %News+TED + WL &26.92& 28.97\\
    \hline
    \multicolumn{3}{c}{Embedding based Methods}\\
    \hline
    MTL & 26.90& 29.27\\
    AdvL  & 25.68& 27.46\\
    PAdvL& 27.06& 29.49\\
    %Partial Adv. + WL& 26.39& 28.52\\
    WDC + WL& 27.25 & 29.43\\
    \hline
    \multicolumn{3}{c}{Our Domain Mixing Methods}\\
    \hline
    Encoder & \textbf{27.78}& 30.30\\
    Encoder + WL & 27.67& 30.11\\
    E/DC & 27.58 & \textbf{30.33} \\
    E/DC + WL& 27.55& 30.22\\
    \hline
    \end{tabular}
     \vspace{-0.05in}
    \caption{English-to-German.}
     \vspace{-0.25in}
    \label{tab:en2deExp}
\end{table}

\begin{figure}[!htb]
    \centering
    \vspace{-0.075in}
    \includegraphics[width=0.6\textwidth]{figure/ppl.pdf}
    \vspace{-0.15in}
    \caption{Perplexity v.s. Number of epochs for English-to-German.}
    \label{fig:en2dePPL}
    \vspace{-0.125in}
\end{figure}

We also compare the perplexity on the validation set in Figure~\ref{fig:en2dePPL}. As can be seen, our domain mixing methods converge faster than the baselines and all methods converge after 50 epochs. We also observe that the baselines get stuck at plateaus at the early stage of training. The possible reason is that their training enforces one unified model to fit data from two different domains simultaneously, which is computationally more difficult. 
%Since different domain may have different optimal parameters, the solution thus keeps wandering around. 
%Though these baselines eventually escape the bad optima, such a pattern is never desired. 
%Each part of the mixing model converges to its own domain optima, and we can reconstruct the model by leveraging the domain proportion and each individual optimal part. 

Table~\ref{tab:en2frExp} shows the BLEU scores of the baselines and our domain mixing methods for English-to-French translation. Note that though the data from the Medical and TED domains are slightly imbalanced (about 1:2.5), our methods can still outperform the baselines on both domains. 


%For the English-to-French task, the mixing methods outperform the other baselines as Table~\ref{tab:en2frExp} shows. Notice that, different from the English-to-German task, the dataset domains are imbalanced. The number of labeled sentences in the Medical domain is twice as many as that of the TED domain . This imbalanced pattern may affect the estimation of the domain proportion. As can be seen in the table, the mixing methods are still valid under slightly imbalance ratio. However, it might be difficult to obtain predictable performance for extreme ratio like $1:10$. In that case, we may need an adaptive algorithm to handle the imbalance issue. We will leave this for future study. 

\begin{table}[!hbt]
%    \small
    \centering
    \vspace{-0.05in}
    \begin{tabular}{c|c|c}
    \hline
    Method & TED & Medical  \\
    \hline
    \hline
    \multicolumn{3}{c}{Direct Training}\\
    \hline
    TED & 28.22& 7.32\\
    Medical & 7.03& 53.73\\
    Medical + TED & 39.21& 53.40\\
    %Medical + TED + WL& 41.16& 55.22\\
    \hline
    \multicolumn{3}{c}{Embedding based Methods}\\
    \hline
    MTL & 39.14& 53.37\\
    AdvL  & 39.54& 53.46\\
    PAdvL& 39.56& 53.23\\
    %Partial Adv. + WL& & \\
    WDC + WL&39.79 &53.85  \\
    \hline
    \multicolumn{3}{c}{Our Domain Mixing Methods}\\
    \hline
    Encoder & 40.30& 54.05\\
    Encoder + WL & 40.43& 54.14\\
    E/DC & 40.52&	54.28 \\
    E/DC + WL & \textbf{40.60} &	\textbf{54.39} \\
	    \hline
	    %E/DC+Adv+WL & 40.55 & 54.26 \\
	    %E/DC+Adv & 40.60 & 54.32 \\
    \end{tabular}
    
    \vspace{-0.1in}
    \caption{English-to-French.}
    \vspace{-0.15in}
    \label{tab:en2frExp}
\end{table}


\begin{table}[!hbt]
    \vspace{-0.05in}
%	\small
	\centering
	\begin{tabular}{c|c|c|c|c}
	    \hline
		Method & Laws & News & Speech & Thesis   \\
		\hline
		\hline
		\multicolumn{5}{c}{Direct Training}\\
		\hline
		Laws &  51.98&	3.80&	2.38&	2.64\\
		News &  6.88&	31.99&	8.12&	4.17\\
		Speech &  3.33&	4.90&	18.63&	3.08\\
		Thesis &  5.90&	5.55&	4.77&	11.06\\
		Mixed &  48.87&	26.92&	16.38&	12.09\\
		%Mixed + WL & 48.63&  27.01&  16.13& 12.17\\
		\hline
		\multicolumn{5}{c}{Embedding based Methods}\\
		\hline
		MTL & 49.14&	27.15&	16.34&	11.80\\
		AdvL  & 48.93&	26.51&	16.18&	12.08\\
		PAdvL & 48.72&	27.07&	15.93&	\textbf{12.23}\\
		%PAdv. + WL& & &  &  \\
		WDC + WL& 42.16& 25.81& 15.29& 10.14\\
		\hline
		\multicolumn{5}{c}{Our Domain Mixing Methods}\\
		\hline
		Encoder & 50.21&	27.94&	16.85&	12.03\\
		Encoder + WL & 50.11& 27.48&	16.79& 11.93\\
		E/DC &\textbf{50.64}&	\textbf{28.48}&	17.41&	11.71  \\
		E/DC + WL & 50.04& 28.17&  \textbf{17.60}& 11.59\\
	    \hline 
	\end{tabular}
	\caption{Chinese-to-English.} 
	\label{tab:zh2enExp_stable}
\end{table}

Table~\ref{tab:zh2enExp} shows the BLEU scores of the baselines and our domain mixing methods for Chinese-to-English translation. As can be seen, our methods outperform the baselines on all domains except Thesis. We remark that the translation for the Thesis domain is actually very difficult, and all methods obtain poor performance.

Moreover, we find that for Chinese-to-English task, all our baselines are sensitive to the architecture of the Transformer. Their training will fail, if we place the layer normalization at the end of each encoder and decoder layer (as \citet{vaswani2017attention} suggest). Therefore, we move the layer normalization to their beginnings. Surprisingly, our domain mixing methods are very stable regardless of the position of the layer normalization. More details can be found in Table~\ref{tab:zh2enExp} of Appendix~\ref{sec:extraexp}.


\vspace{-0.075in}
\subsection{Ablation Study}
\vspace{-0.075in}

We further shows that the performance gains are from the domain mixing methods, instead of from the increased model capacity. Table~\ref{tab:ablationExp} shows the BLEU scores with and w/o using domain labels under equal model size. We keep the model size consistent by adopting the same network structure and the same number of parameters as in the domain mixing methods. The only difference is that we remove domain label to guide the training of domain proportion, i.e., only $L_{\rm gen}$ is used in the training loss, and $L_{\rm mix}$ is removed. Training w/o domain labels shows a slight improvement over baseline, but is still significantly worse than our proposed method for most of the tasks. Therefore, we can conclude that our proposed domain mixing approach indeed improves performance.

\begin{table}[!hbt]
	\vspace{-0.05in}
%	\small
	\centering
	\begin{tabular}{c|c|c|c}
		\hline
		Method & Direct Training & w/o DL & with DL (Ours)  \\
		\hline
		\hline
		\multicolumn{4}{c}{English-to-Germany}\\
		\hline
		News &  26.06 &	26.25 &	\textbf{27.78}\\
		TED & 28.11 & 28.27 & \textbf{30.30} \\
		\hline
		\multicolumn{4}{c}{English-to-French}\\
		\hline
		TED & 39.21 & 39.39 & \textbf{40.30} \\
		Medical & 53.40 & 53.33 & \textbf{54.05} \\
		\hline
		\multicolumn{4}{c}{Chinese-to-English}\\
		\hline
		Laws & 48.87 & 48.96 & \textbf{50.21} \\
		News & 26.92 & 27.02 & \textbf{27.94} \\
		Speech & 16.38 & 16.15 & \textbf{16.85} \\
		Thesis & \textbf{12.09} & 12.03 & 12.03 \\
		\hline 
	\end{tabular}
	\caption{BLEU Scores with and w/o domain labels (DL) under equal model capacity.} 
	\label{tab:ablationExp}
\end{table}
\vspace{0.1in}


\vspace{-0.075in}
\subsection{Visualizing Domain Proportions} \label{sec:exp_domainprop}
\vspace{-0.075in}

To further investigate our domain mixing methods, we plot the domain proportions of the word embedding at different layers. A uniform proportion, e.g., $(0.5,0.5)$, is encouraging knowledge sharing across domains, while a skewed proportion, e.g., $(0.1,0.9)$, means there is little knowledge to share across domains.%, since the embedding contains a lot of domain specific information and/or the meaning of the word is well understood.
\begin{figure}[htb!]
	\centering
	\includegraphics[width=0.7\textwidth]{figure/domain_prop/explain.png}
	\caption{Domain proportion of a sentence from the TED domain for English-to-French task. The domain proportion is extracted from all layers of the encoder.} 
	\label{fig:explain}
\end{figure}
Figure~\ref{fig:explain} illustrates how the knowledge sharing is controlled via the domain proportion. The selected sentence is from the English-to-French task, containing TED and Medical domains. Specifically, we observe :

\smallskip

%We observe the following facts that help us understand the knowledge sharing across the domains:\\
\noindent $\bullet$ The domain proportions of different words at different layers have various patterns.

\smallskip

\noindent $\bullet$ At the bottom layers, the domain proportion of a word is closely related to its frequency of occurrence.

\smallskip

%For example, \textit{we} is more likely to occur in TED domain, since the medical domain contains many professional publications, which are usually written in the third person.\\
\noindent $\bullet$ Some words with simple semantic meanings do not need to borrow much knowledge from other domains, e.g., \textit{and}; Some other words need to borrow knowledge from other domains to better understand their own semantic meaning. For example, the word \textit{phenomenon} keeps borrowing/sharing knowledge from/to the medical domain at every layer.

\smallskip

\noindent $\bullet$ The ending of the sentence only conveys a stopping signal, and thus is shared across all domains.

\smallskip

\noindent $\bullet$ The domain proportions at the bottom layers tend to be more diverse, while those at the top layers tend to be more skewed, as shown in Figure~\ref{fig:domainprop_senence} for English-to-German task.

\smallskip

\noindent $\bullet$  The domain proportions of the decoder tend to be more skewed than those of the encoder, which demonstrates little knowledge sharing. Figure~\ref{fig:domainprop_hist} shows the histograms of word-level domain proportions at different layers in both the encoder and decoder. This might explain why the mixing decoder only contributes limited performance gain for the English-to-German task. 
% For the same reason, the weighted loss proposed in \citet{zeng2018multi} can be less effective for the Transformers, since every single position of the last hidden representation in the decoder already has very clear domain information. 



%As can be seen in Figure~\ref{fig:domainprop_senence} and Figure~\ref{fig:domainprop_hist}, the word-level domain portion is very diverse in the lower layers of the encoder. That is because, without knowing much about the context, their semantic meaning is more neutral. The mixing model benefits the translation by adaptively captures the world-level domain information. In the higher level, the word embedding will have clear domain information based on the context. Hence, there will be less sharing. That explains why incorporating the mixing decoder only obtains limited gain and even hurts the performance for the English-to-German task.

\begin{figure}[htb!]
	\centering
%	\vspace{-0.05in}
	\includegraphics[width=0.7\textwidth]{figure/domain_prop/en2de/prop.png}
%	\vspace{-0.15in}
	\caption{Domain proportions of a sentence pair for English-to-German task. White represents the News domain and black represents the TED domain. The domain proportions of both the encoder (bottom) and the decoder (top) are presented. } 
%	\vspace{-0.15in}
	\label{fig:domainprop_senence}
\end{figure}

\begin{figure}[htb!]
%\vspace{-0.1in}
\centering
	\begin{tabular}{cccccc}
		Layer-1 &2&3&4&5&6\\
		\hline
		\includegraphics[width=0.13\textwidth]{figure/domain_prop/en2de/encoder_layer0.pdf}&
		\includegraphics[width=0.13\textwidth]{figure/domain_prop/en2de/encoder_layer1.pdf}&
		\includegraphics[width=0.13\textwidth]{figure/domain_prop/en2de/encoder_layer2.pdf}&
		\includegraphics[width=0.13\textwidth]{figure/domain_prop/en2de/encoder_layer3.pdf}&
		\includegraphics[width=0.13\textwidth]{figure/domain_prop/en2de/encoder_layer4.pdf}&
		\includegraphics[width=0.13\textwidth]{figure/domain_prop/en2de/encoder_layer5.pdf} \vspace{-0.1in}\\
		\multicolumn{6}{c}{Encoder} \\
		\includegraphics[width=0.13\textwidth]{figure/domain_prop/en2de/decoder_layer0.pdf}&
		\includegraphics[width=0.13\textwidth]{figure/domain_prop/en2de/decoder_layer1.pdf}&
		\includegraphics[width=0.13\textwidth]{figure/domain_prop/en2de/decoder_layer2.pdf}&
		\includegraphics[width=0.13\textwidth]{figure/domain_prop/en2de/decoder_layer3.pdf}&
		\includegraphics[width=0.13\textwidth]{figure/domain_prop/en2de/decoder_layer4.pdf}&
		\includegraphics[width=0.13\textwidth]{figure/domain_prop/en2de/decoder_layer5.pdf} \\
		\multicolumn{6}{c}{Decoder} \\
	\end{tabular}
\caption{Histograms of the domain proportions of each layer in our domain mixing model for English-to-German Task. Within each histogram, $0$ means pure News domain, and $1$ means pure TED domain.} 
%	\vspace{-0.1in}
\label{fig:domainprop_hist}
\end{figure}


%\textbf{Weight Loss}
% We observe that in some scenario only applying the mixing to the encoder is sufficient to obtain a better result. Section~\ref{sec:exp_domainprop} further discusses the reason why a mixing decoder only slightly benefits the training.  



\vspace{-0.05in}
\subsection{Combining Domain Mixing with Domain Aware Embedding}\label{sec:grad_flow}
%\vspace{-0.05in}

The embedding based methods can be naturally combined with our domain mixing methods. As we mentioned in \ref{sec:implementation_details}, the domain proportion is trained solely, meaning gradient does not propagate between the domain proportion layers $\cD$ and the Transformer. The computation of the gradient, on the other hand, is the key to combining two methods. Specifically, we encourage the embedding to be domain aware via MTL, AdvL and PAdvL, where we use the domain proportion layers to guide the training of the embedding. Figure~\ref{fig:mix_embed} illustrates the back-propagation under different methods. Table~\ref{tab:zh2enExp_mixembed} shows the performance for Chinese-to-English task under this setting. Here we consider applying domain mixing only to the encoder as the baseline. As can be seen, by applying appropriate domain aware embedding, the performance can be further improved.

%The domain proportion layers $\cD$ are only used for estimating the domain proportion and should not intervene in the training of the translation model. So the gradient propagation is cut off between the Transformer and the domain proportion as Figure~\ref{fig:detached_train} shows. More discussion about the training procedure can be found in Section~\ref{sec:grad_flow}

\begin{figure}
		\centering
	\begin{tabular}{c}
		\includegraphics[width=0.7\textwidth]{figure/gradientflow.png}
	\end{tabular}
	\caption{Back-propagation for different embedding based methods.} 
	\label{fig:mix_embed}
\end{figure}

\begin{table}[!hbt]
%	\small
	\centering
	\begin{tabular}{c|c|c|c|c}
	    \hline
		Method & Laws & News & Speech & Thesis   \\
		\hline
		\hline
		Encoder & 50.21&	27.94&	16.85&	12.03\\
		+MTL & 49.15 & 26.82 & 15.72 & 11.93 \\
		+Adv &50.18 & 27.72 & \textbf{16.99} & \textbf{12.16}\\
		+PAdvL &49.01	& 26.63	& 16.06	& 12.15 \\
		+Multitask + WL&48.75 & 26.78 & 16.53 & 12.11\\
		+Adv + WL&\textbf{50.24}&	\textbf{28.21}&	16.98&	12.00\\
		+PAdv + WL & 48.87 & 26.86 & 16.14 & 11.89\\
		\hline
		%Both+Adv + WL & 50.00&	28.46&	17.68&	11.54\\
	    %\hline
	\end{tabular}
	\caption{BLEU Scores of Domain Mixing + Domain Aware Embedding for Chinese-to-English Task} %(Stable version by putting layer norm before attention)}
	\label{tab:zh2enExp_mixembed}
\end{table}


==> tech report/introduction.tex <==
%!TEX root = ./acl2019.tex

\vspace{-0.1in}
\section{Introduction} \label{sec:intro}
\vspace{-0.1in}

%Many efforts have been devoted to studying 
%is an end-to-end approach that uses a single integrated deep neural network-based model to predict the likelihood of entire sentences (sequences of words), and 
Neural Machine Translation (NMT) has made significant progress in various machine translation tasks \citep{kalchbrenner2013recurrent,sutskever2014sequence,bahdanau2014neural,luong2015effective,wu2016google}. 
The success of NMT heavily relies on a huge amount of annotated parallel sentences as training data, which is often limited in certain domains, e.g., medical domain.  One approach to address this is to explore unparalleled corpora, such as unsupervised machine translation~\citep{lample2017unsupervised,lample2018phrase}. Another approach is to train a multi-domain NMT model and this is the focus of this paper. The simplest way is to build a unified model by directly pooling all training data from multiple domains together, as the languages from different domains often share some similar semantic traits, e.g., sentence structure, textual style and word usages. For domains with less training data, the unified model usually shows significant improvement. %in the translation performance.


Researchers have proposed many methods for improving multi-domain NMT. Though certain semantic traits are shared across domains, there still exists significant heterogeneity among languages from different domains. For example, \citet{haddow2012analysing} show that for a domain with sufficient training data, a unified model may lead to weaker performance than the one trained solely over the domain; \citet{farajian2017neural,luong2015effective,sennrich2015improving,servan2016domain} also show that to improve the translation performance over certain domains, fine-tuning the unified model is often needed, but at the expense of sacrificing the performance over other domains. This indicates that a unified model might not well exploit the domain-specific knowledge for each individual domain. %, causing degraded performances in each constituent domain.

To overcome this drawback, two lines of recent research focus on developing new methods by exploiting domain-shared and domain-specific knowledge to improve multi-domain NMT \citep{britz2017effective,zeng2018multi,tars2018multi,hashimoto2016domain, wang2017instance,chen2017cost,wang2018sentence}.  

One line of research focuses on instance weighting, which assigns domain related weights to different samples during training. For example, \citet{wang2017instance} consider sentence weighting and domain weighting for NMT. The sentence weight is determined by the bilingual cross-entropy of each sentence pair based on the language model of each domain. The domain weight can be modified by changing the number of sentences from that domain in a mini-batch. \citet{chen2017cost} propose a cost weighting method, where the weight of each pair of sentences is evaluated by the output probability of a domain classifier on the encoder embedding. \citet{wang2018sentence} propose a dynamic training method to adjust the sentence selection and weighting during training. We remark that many of these methods are complementary to our proposed model, and can be applied to improve the training of our model.

Another line of research attempts to design specific encoder-decoder architectures for NMT models. For example, \citet{britz2017effective} consider domain-aware embedding given by the encoder, and then jointly train a domain classifier, taking the embedding as input to incorporate the domain information. \citet{zeng2018multi} further extend their approach by separating the domain-shared and domain-specific knowledge within the embedding. In addition, \citet{zeng2018multi} and \citet{shen2018word} propose a maximum weighted likelihood estimation method, where the weight is obtained by word-level domain aware masking to encourage the model to pay more attention to the domain-specific words. The aforementioned methods, however, have a notable limitation: They enforce one single encoder to learn shared embedding across all domains, which often lacks adaptivity to each individual domain. 
%They only focus on learning the shared embedding , which lacks flexibility for capturing domain-specific knowledge.

%which has limitations for multi-domain NMT
%
%improves The embedding, however, exploiting 
%
% However, improving multi-domain NMT solely based on the embedding
%
%, however, is very limited.
%
%
%The aforementioned methods only focus on improving the embedding in .
%
%however, have limitations 


%NEED TO TALK ABOUT LIMITATIONS?(i.e. These proposed models rely solely on the information encoded in domain aware embeddings, yet ignoring different rules for building models in different domains. Our proposed method will tackle this issue by leveraging information from multi-realizations of model space.)

%These methods mainly fall into two categories: (1) Some research propose general domain adaptation techniques to machine translation, such as instance reweighting and data selection. 

To better capture domain-shared knowledge beyond shared embedding from a single encoder, we propose a novel multi-domain NMT model using individual modules for each domain, on which we apply word-level, adaptive and layer-wise domain mixing. 
%Our proposed model is motivated by the observation that every word will have its own domain proportion. If a word is common in different domains, the knowledge can be shared across them. For instance, the word ``article'' appears in the domains of laws and business. Therefore, we expect the knowledge for translating the word ``article'' to be shared between these two domains. If a word is specific for one domain, we do not need to share the knowledge across other domains and just make it as domain-specific knowledge. The other domains, however, can still borrow the knowledge when needed. For instance, the word ``phenomenon'' always appears in scientific domain, while it is rarely used in spoken language. To understand a sentence from speech domain, which contains ``phenomnon'', we want to borrow knowledge from scientific domain for this specific word while for the other part we still need to maintain the textual style of the spoken language. To achieve the above adaptivity, our proposed model assigns a context-dependent domain proportion\footnote{A word actually has multiple domain proportions at different layers of our model. See more details in Section 3} to every word in the sentence. Therefore, we carefully design multi-head dot-product attention modules for different domains, and eventually mix these modules by taking weighted averages of their parameters by their layer-wise domain proportions.
Our proposed model is motivated by the observation that although every sentence of the training data has a domain label, the words in the sentence are not necessarily only related to that domain. For instance, the word ``article'' appears in the domains of laws and business. Therefore, we expect the knowledge for translating the word ``article'' to be shared between these two domains. 
Our proposed model assigns a context-dependent domain proportion\footnote{A word actually has multiple domain proportions at different layers of our model. See more details in Section 3} to every word in the sentence. The domain proportions of the words can be naturally integrated into the Transformer model for capturing domain-shared/specific knowledge, as the multi-head dot-product attention mechanism is applied at the word-level. Specifically, we carefully design multi-head dot-product attention modules for different domains, and eventually mix these modules by taking weighted averages of their parameters by their layer-wise domain proportions.

Compared with existing models, ours has the following two advantages: %\todo{This following two bullets are somehow overlapped?}

\smallskip

\noindent $\bullet$ Our proposed model is more powerful in capturing the domain-specific knowledge, as we design multiple dot-product attention modules for different domains. In contrast, existing models rely on one single shared encoder, and then one single unified translation model is applied, which often cannot adapt to each individual domain very well.

\smallskip

\noindent $\bullet$ Our proposed model is more adaptive in the process of domain knowledge sharing. For common words across domains, their domain proportions tend to be uniform, and therefore can significantly encourage knowledge sharing. For some words specific to certain domains, their domain proportions tend to be skewed, and accordingly, the knowledge sharing is encouraged only within the relevant domains. For example, the word ``article'' appears less in the medical domain than the domains of laws and business. Therefore, the corresponding domain proportion tends to favor the domains of laws and business more than the medical domain.

\smallskip

We evaluate our proposed model in several multi-domain machine translation tasks, and the empirical results show that our proposed model outperforms existing ones and improves the translation performance for all domains.

%
%
%\textbf{Paragraph 3: In this paper we propose, XXXX.}
%An NMT model essentially captures the translation generating process from the source language to the target language. Different domains will certainly have different generating process, i.e., relying on different NMT models. All previous researches, however, tries to use one unified model to capture the heter. 
%In this paper, we incorporate domain knowledge into NMT models via multihead-attention based domain-aware word-level parameter mixing. Specifically, every word is associated with a mixture of domains, which can be recongnized as domain prior. The mixing of sub-models is based on the prior.   
%%The mixture is represented by a domain prior, which is sampled from a Dirichlet distribution. The observed domain labels of the training data can be considered as realizations of categorical distribution based on the domain prior. Because of the latent domain mixture prior, we do not directly associate tranlation models to specific domain labels. Instead we associate the model with the domain prior. We further derive fast approximation for latent variable inference, parameter estimation, and prediction. 
%
%
%
%An NMT model essentially captures the translation generating process from the source language to the target language. Different domains will certainly have different generating process, i.e., relying on different NMT models. All previous researches, however, only focusing on one unified model. Inspired by latent Dirichlet allocation (LDA), we propose a domain-aware Bayesian NMT model. More precisely, XXXXXXXXXXXXXXX. 
%
%\textbf{Paragraph 3: Our result and contributions.} XXXXXXXXXXXXX. Our model is more flexible and powerful and can automatically capture domain-share and domain-specific knowledge from the model space. 

%The rest of the paper is organized as follows: Section~\ref{sec:background} briefly reviews the background; Section ~\ref{sec:method} presents our proposed word-level adaptive domain mixing NMT model; Section~\ref{sec:exp} presents numerical experiments on English-German, English-French, Chinese-English multi-domain datasets; Section~\ref{sec:relatedwork} discuss related works and draw a brief conclusion. 


%\textbf{Related Literature}
%These researches are focusing on the same topic and are the most relevent: \cite{britz2017effective,zeng2018multi,wang2018sentence,tars2018multi,hashimoto2016domain}.
%This one \citep{chu2018survey} is a very comprehensive literature review of domain adaptation of MT.

==> tech report/methodology.tex <==
%!TEX root = ./acl2019.tex


\vspace{-0.1in}
\section{Model} \label{sec:method}
\vspace{-0.1in}

We present our Transformer-based multi-domain neural machine translation model with word-level layer-wise domain mixing.

\vspace{-0.075in}
\subsection{Domain Proportion}\label{sec:domainprop}
\vspace{-0.075in}

Our proposed model is motivated by the observation that although every sentence in the training data has a domain label, a word in the sentence does not necessarily only belong to that single domain. Therefore, we assume that every word in the vocabulary has a domain proportion, which indicates its domain preference. Specifically, given the embedding $x\in\RR^{d}$ of a word, $k$ domains and $R\in\RR^{k\times d}$, our model represents the domain proportion by a smoothed softmax layer as follows, 
\begin{align*}
\cD(x) = (1-\epsilon)\cdot\textrm{softmax}(Rx)+\epsilon/k,
\end{align*}
where $\epsilon\in(0,1)$ is a smoothing parameter to prevent the output of $\cD(x)$ from collapsing towards $0$ or $1$. Specifically, setting $\epsilon$ as a large value encourages the word to be shared across domains.

\vspace{-0.075in}
\subsection{Word-Level Adaptive Domain Mixing}\label{sec:word_level_mixing}
\vspace{-0.075in}

In our proposed model, each domain has its own multi-head attention modules. Recall that the point-wise linear transformations in the multi-head attention module $W_{i,Q}$'s, $W_{i,K}$'s, $W_{i,V}$'s and $W_O$ are applied to each word separately and identically, as shown in Figure~\ref{fig:pointwiselinear}.
\begin{figure}[!htb]
\centering
\vspace{-0.2in}
\includegraphics[width=0.3\textwidth]{figure/pointwiselinear}
\vspace{-0.1in}
\caption{The Point-wise Linear Transformations are applied at the word-level.}
\vspace{-0.15in}
\label{fig:pointwiselinear}
\end{figure}
Therefore, we can naturally integrate the domain proportions of the words with these multi-head attention modules. Specifically, we take the weighted averaging of the linear transformation based on the domain proportion $\cD(x)$. For example, we consider the point-wise linear transformations $\{W_{i,Q,j}\}_{j=1}^k$ on the $t$-th word of the input, $Q_t$, of all domains. The mixed linear transformation can be written as 
\[
\textstyle\overline{Q}_{i,t}=\sum_{j=1}^k Q_t^\top W_{i,Q,j} \cD_{Q,j}(Q_t),
\]
where $\cD_{Q,j}(Q_t)$ denotes the $j$-th entry of $\cD_Q(Q_t)$, and $\cD_Q$ is the domain proportion layer related to $Q$. Then we only need to replace $\tilde{Q}_i$ in \eqref{MHT} with
\begin{align*}[\overline{Q}_{i,1},...,\overline{Q}_{i,n}].
\end{align*}
%Similarly, we can obtain $\tilde{K}_i$, $\tilde{V}_i$ and $H_i$ in \eqref{MHT}. 
An illustrative example is presented in Figure~\ref{fig:mixlinear}. For other linear transformations, we applied the domain mixing scheme in the same way.
\begin{figure}[!htb]
	\centering
	\vspace{-0.1in}
	\includegraphics[width=0.45\textwidth]{figure/wordlevelmix.png}
	\vspace{-0.1in}
	\caption{Word-level mixing with 3 domains. For simplicity, we omit the subscripts $Q,i$.}
	\vspace{-0.1in}
	\label{fig:mixlinear}
\end{figure}
We remark that the Transformer model, though does not have any explicit recurrent structure, handles the sequence through adding additional positional embedding for each word (in conjunction with sequential masking). Therefore, if a word appears in different positions of a sentence, its corresponding embedding is different. This indicates that the domain proportions of the same word can also be different across positions. This feature makes our model more flexible, as the same word in different positions can carry different domain information.

%Therefore, we only need to design multiple dot-product attention modules for different domains, and eventually mix these modules by taking weighted averages of their parameters by the domain proportion of the word. 

%$\cD(\xb)$ maximizes the predicted probability of the correct domain class label $d$ conditioned on the $\xb$ by minimizing 
%\begin{align}
%\cL_{disc} = \ell(\cD(\xb),d),
%\end{align}
%where $d$ is the domain label, $\ell$ is the negative cross-entropy loss.
%The translation model is trained together with the domain discriminator as Figure~\ref{fig:general_model} shows. In this we consider two training schemes: \\
%\noindent $\bullet$ Joint training allows the discriminator supervise the training of embedding. On the other hand, the translation model can also supervise the training of the discriminator. \\
%\noindent $\bullet$ Detached training means the domain discriminator is trained solely. The translation model only takes the domain proportion as a fixed input. \\
%
%\begin{figure}[!ht]
%	\centering
%	\includegraphics[width=0.4\textwidth]{figure/model.png}
%	\caption{Domain Mixing}
%	\label{fig:general_model}
%\end{figure}

\vspace{-0.075in}
\subsection{Layer-wise Domain Mixing}\label{sec:layerwise}
\vspace{-0.075in}

Recall that the Transformer model contains multiple multi-head attention modules/layers. Therefore, our proposed model inherits the same architecture and applies the word-level domain mixing to all these attention layers. Since the words have different representations at each layer, the corresponding domain proportions at each layer are also different, as shown in Figure \ref{fig:fullmodel}. In addition to the multi-head attention layers, we also apply similar word-level domain mixing to the point-wise two-layer fully connected feed-forward network.

The layer-wise domain mixing allows the domain proportions to be context dependent. This is because the domain proportions are determined by the word embedding, and the word embedding at top layers is essentially learnt from the representations of all words at bottom layers. As a result, when the embedding of a word at some attention layer is already learned well through previous layers (in the sense that it contains sufficient contextual information and domain knowledge), we no longer need to borrow knowledge from other domains to learn the embedding of the word at the current layer. Accordingly, the associated domain proportion is expected to be skewed and discourages knowledge sharing across domains. This makes the process of knowledge sharing of our model more adaptive.


%for the same word, the embedding is context dependent.

%The layer-wise domain mixing allows the domain proportion to be context dependent. This is because for the same word, the embedding is context dependent. 

%our model to. This is because for the same word, the embedding is context dependent. And accordingly, the domain proportion is also context dependent. With different level 0f contextual information in different layers, the knowledge sharing is adaptively controlled by the context dependent domain proportion. For example, with more contextual information in the top layers, the domain proportion tends to be skewed and encourage knowledge sharing/borrowing from/to targeted domains.



\begin{figure}[!htb]
	\centering
	\vspace{-0.25in}
	\includegraphics[width=0.45\textwidth]{figure/fullmodel}
	\vspace{-0.15in}
	\caption{Illustration of Our Multi-domain NMT Model: Normalization and residual connection are omitted for simplicity. For all other detail, please refer to \citet{vaswani2017attention}. }
	\vspace{-0.2in}
	\label{fig:fullmodel}
\end{figure}


\vspace{-0.05in}
\subsection{Training} \label{sec:training}
\vspace{-0.05in}

Recall that $\cH$ denotes the encoder, $\cF$ denotes the decoder, and $\cD$ denotes the domain proportion. Define $\Theta=\{\cF,\cH,\cD\}$. The proposed model can be efficiently trained by minimizing a composite loss function defined as follows,
\begin{align*}
L^* = L_{\rm gen}(\Theta) + L_{\rm mix}(\Theta),
\end{align*}
where $L_{\rm gen}(\Theta)$ denotes the cross-entropy loss over the training data $\{\xb_i, \yb_i\}_{i=1}^n$, and $L_{\rm mix}(\Theta)$ denotes the cross entropy loss over the words/domain (hard) labels.

For $L_{\rm mix}(\Theta)$, the domain labels are obtained from the training data. Specifically, for all words in a sentence belonging to the $J$-th domain, we specify their domain hard labels as $J$. Then given the embedding $x$ of a word, we compute the cross entropy loss of its domain proportion $\cD(x)$ as $-\log(\cD_J(x))$. Accordingly, $L_{\rm mix}(\Theta)$ is the sum of the cross entropy loss over all such pairs of word/domain label of the training data.



%\subsection{Connection to Generative Models}
%
%Our proposed model is related to the following data generating process: Given some $x\in\RR^{d}$ and $U\in\RR^{k\times d}$ and $V_j\in\RR^{v\times d}$, where $d$ is the size of vocabulary, we have
%
%\smallskip
%
%$\bullet$ $\theta\sim \mathrm{Dir}(\mathrm{softmax}(Ux))$;
%
%\smallskip
%
%$\bullet$ $C\sim\mathrm{Multinomial}(\theta)$;
%
%\smallskip
%
%$\bullet$  $y\sim\mathrm{Multinomial}(\mathrm{softmax}(\sum_{j=1}^k\theta_j\cdot V_jx))$.
%
%\smallskip
%
%\noindent Roughly speaking, the above generating process can be viewed as a highly simplified multi-domain machine translation model for one single word: $x$ denotes the embedding of the input word, $\theta$ is the domain proportion of the word, $C$ denotes the domain hard label, and $y$ denotes the output word. For multiple words, our proposed model is more complicated and .%As can be seen, the domain proportion is essentially the weight for averaging the translation model from different domains.
%

%\vspace{-0.075in}
%\subsection{Connection to Word Disambiguation}
%\vspace{-0.075in}
%
%One major challenge in multi-domain machine translation is the word ambiguity in different domains. For example, the word ``article'' has different meanings in the domains of laws and media. When translating ``article" into Chinese, the translated words are \begin{CJK*}{UTF8}{gbsn}
%``条款''
%\end{CJK*} and \begin{CJK*}{UTF8}{gbsn}
%``文章''
%\end{CJK*}, meaning a separate clause of a legal document and a piece of writing. Our proposed word-level layer-wise domain mixing approach tends to reduce the word ambiguity. As mentioned in Section~\ref{sec:layerwise}, our model extracts different representations of each word from contexts at different layers. Accordingly, the domain proportion of each word evolves from bottom to top layers, and can eventually help identify the corresponding domains.
%
%\begin{table}[!htb]
%	\small
%	\centering
%	\vspace{-0.1in}
%		\begin{tabular}{ c|c } 
%			\hline
%			\multirow{2}{*}{Laws} & ``\textbf{Article} 37 The freedom of marriage ...'' \\
%			& \begin{CJK*}{UTF8}{gbsn}
%				``第三十七\textbf{条}:婚姻的自由 ...''
%			\end{CJK*} \\
%		\hline
%		\multirow{2}{*}{Media}& ``... working on an \textbf{article} about the poems ...'' \\
%		& \begin{CJK*}{UTF8}{gbsn}
%			``... 为了一篇诗的\textbf{文章} ...''
%		\end{CJK*}\\
%	\hline
%		\end{tabular}
%	\vspace{-0.05in}
%\caption{The ambiguity of ``articles''.}
%\vspace{-0.15in}
%\end{table}
%
%Moreover, as mentioned in Section~\ref{sec:word_level_mixing}, the positional embedding also contributes to the word disambiguation in multi-domain translation. For example, in the law domain, we find that ``article'' often appears at the beginning of a sentence, while in the media domain, the word ``article'' may appear in other positions. Therefore, varying domain proportions for different positions can help with word disambiguation.
%
%We remark that word disambiguation across domains actually requires $\cD(x)$ to be powerful for predicting the domain of the word. However, a powerful $\cD(x)$ tends to yield skewed domain proportions and is not flexible enough for domain knowledge sharing. To trade off between strength and flexibility of $\cD(x)$, the smoothing parameter $\epsilon$ of $\cD(x)$ (see Section~\ref{sec:domainprop}) needs to be properly set.

%\textbf{Remark 2} The number of parameters grows as the number of domains increases. In practice, we can aggregate similar domains into one domain to prevent the model from growing too large. More discussion regarding the number of parameters is in section~\ref{sec:exp}.
%
%
%
%\subsection{Extension: Bayesian}
%We 
%
%
%
%\subsection{title}
%
%We first consider a general parametric model, 
%$f(x;\theta) $, where $x$ is the input and $\theta$ is the parameter. Multi-domain dilemma is that when the model is trained over one single domain, it will perform poorly on other domains. If we know which domain $x$ comes from, we can build an individual model $f_d(\cdot;\theta_d)$ for each domain $D_d$ and then assign $x \in D_d$ to the corresponding model $f_d(\cdot;\theta_d)$. However, obtaining the domain label is not possible when serving the model. To address this issue, people usually train a unified the model over multiple domains, the performance, however, will sometimes be degenerated for each individual domain \cite{britz2017effective}. So how to build a unified model without performance degradation, or even improve it by utilizing the information from all domains becomes a problem. 
%
%\subsection{Domain Aware Bayesian Approach} 
%
%In Bayesian statistics, the parameters $\theta$ is not deterministic but follows some distribution. In the multi-domain setting, we assume $\theta$ is depending on the domain $D$ of $x$ as  shows.
%
%Notice that each time the model use the expectation of the $\hat{\theta}(x)=\EE_{\theta|D(x)}[\theta]=\sum_dD_d(x)\theta_d$ as the model parameter for the given input $x$.
%The conditional distribution of $D|x$ is given by a classification model which is denoted by $D(x)$, which outputs a discrete distribution over domains. $D$ can be trained by minimizing the cross entropy loss on the labeled training data:
%\begin{align}
%    \min_D \EE_x [ -\log(D_{d_x}(x))],
%\end{align}
%where $D_{d_x}(x)$ is the $d_x$-th output of $D(x)$, and $d_x$ is the domain label of $x$. This additional classification task can be either trained in a \textbf{detached} way or a \textbf{joint} way with original task. The detached training means when the training $D$ is independent of the training of original task and the gradient will not flows between two tasks. The joint training, on the other hand, allows gradient flows between two task and allows the two training procedure to interact with each other. 
%
%\subsection{Sentence level Bayesian Approach}
%Different from traditional classification and regression task, an NMT model has a more fine-grained and complex structure. Specifically, we consider a word-level, multi-layer NMT, which is denoted as:
%\begin{align}
%    f = f_L \circ f_{L-1} \dotsc \circ f_1,
%\end{align}
%Where $L$ is the number of layers and each layer $f_i$ associate with the parameter $\theta_i$. 
%The input of $f_i$ which is also the output of the $f_{i-1}$ is denoted as $E_i \in \RR^{l \times h_i}$, where $l$ is the length of the sentence and $h_i$ is the dimension of the latent representation. We also call $E_i$ the latent sentence.  
%
%\textbf{Sentence Level Bayesian} When consider the domain label of the latent sentence $E_i$, we can directly train a domain classifier $D_i(E_i)$. So the $i$-th layer with sentence level Bayesian parameter will be $f_i(E_i;\EE_{\theta|D_i(E_i)}(\theta))$.
%
%\textbf{Word-Level Bayesian} If we consider the word-level structure of the model, we can come up with a better mixing strategy. Specifically, each word in the sentence can either comes from an individual domains or is a general word for all domain. As a result, each word will have its own domain information. Like Transformer, many NMT model perform linear operation to each word. This allows us to have a word specific weight, based of the domain information of each word. 
%
%\textbf{Smoothing to a uniform prior} Sometimes a sentence or a word may carry out a very strong domain signal and the classifier $D$ may achieve extremely high accuracy. If the domain classification can exactly recover the domain label of the input, there will be no difference between Bayesian model and ensemble models for every domain. We propose to apply an smoothing technique to explicitly encourage different domain to learn from each other. Specifically, we replace the conditional domain distribution by a smoothed distribution:
%\begin{align}
%    \tilde{D}(x) =  \frac{\epsilon}{\#  \textrm{Domains}}+(1-\epsilon)D(x),
%\end{align}
%where $\epsilon$ is a predefined smoothing parameter.
%
%\subsection{Domain Aware Bayesian Attention} 
%
%
%\textbf{Domain Aware Bayesian Attention} Domain aware Bayesian Attention essentially make the input projection matrices to be sentence/word-level Bayesian weight as illustrated in the right part of Figure~\ref{fig:attention}. 
%
%\begin{figure*}[!ht]
%    \centering
%    \includegraphics[width=0.9\textwidth]{/MultiHeadAtt.pdf}
%    \caption{Multi-head Attention}
%    \label{fig:attention}
%\end{figure*}
